EmoStyle: Emotion-Driven Image Stylization

Art has long been a profound medium for expressing emotions. While existing image stylization methods effectively transform visual appearance, they often overlook the emotional impact carried by styles. To bridge this gap, we introduce Affective Image Stylization (AIS), a task that applies artistic styles to evoke specific emotions while preserving content. We present EmoStyle, a framework designed to address key challenges in AIS, including the lack of training data and the emotion-style mapping. First, we construct EmoStyleSet, a content-emotion-stylized image triplet dataset derived from ArtEmis to support AIS. We then propose an Emotion-Content Reasoner that adaptively integrates emotional cues with content to learn coherent style queries. Given the discrete nature of artistic styles, we further develop a Style Quantizer that converts continuous style features into emotion-related codebook entries. Extensive qualitative and quantitative evaluations, including user studies, demonstrate that EmoStyle enhances emotional expressiveness while maintaining content consistency. Moreover, the learned emotion-aware style dictionary is adaptable to other generative tasks, highlighting its potential for broader applications. Our work establishes a foundation for emotion-driven image stylization, expanding the creative potential of AI-generated art.

==> src/macros.tex <==
% Our packages and commands
%\usepackage{color}
%\usepackage{xcolor}
%\usepackage{graphicx}
%\usepackage{booktabs}
%\let\Bbbk\relax         %%redefined in newtxmath.sty
%\usepackage{amsmath, amsthm, amsfonts, amssymb}
%\usepackage{mathrsfs}
%\usepackage{textcomp}
%\usepackage{epstopdf}
%\usepackage{multirow}
%\usepackage{wrapfig}
%\usepackage{subfig}
%\usepackage{booktabs} % For formal tables
%\usepackage[ruled]{algorithm2e} % For algorithms
% \usepackage{algorithm}
% \usepackage{algorithmic}
% \usepackage[algcompatible]{algpseudocode}
%\usepackage{comment}
%\usepackage{algorithm}  
%\usepackage{algorithmicx}  
%\usepackage{algpseudocode}
%\usepackage{ragged2e}
%\usepackage[normalem]{ulem}
%\usepackage{cleveref}
%\usepackage{bm}
%\usepackage{ulem}
%\usepackage{makecell}
%\usepackage{diagbox}

%\renewcommand{\algorithmcfname}{ALGORITHM}
%\SetAlFnt{\small}
%\SetAlCapFnt{\small}
%\SetAlCapNameFnt{\small}
%\SetAlCapHSkip{0pt}

\newcommand{\N}{\mathcal{N}}
\newcommand{\D}{\hat{\mathcal{D}}}
\newcommand{\F}{\hat{\mathcal{F}}}
\newcommand{\R}{\hat{\mathcal{R}}}

\definecolor{green}{rgb}{0, 0.5, 0}
\definecolor{orange}{rgb}{0.6, 0.3, 0.1}
\definecolor{red}{rgb}{1.0, 0.0, 0.0}
\definecolor{teal}{rgb}{0.0, 0.4, 0.4}
\definecolor{purple}{rgb}{0.65,0,0.65}
\definecolor{saffron}{rgb}{0.95,0.75,0.2}
\definecolor{turquoise}{rgb}{0.0,0.5,0.5}
\definecolor{brown}{rgb}{0.5, 0.16, 0.16}
\definecolor{brickred}{rgb}{.6, .2 .1}
\definecolor{coral}{rgb}{1,0.45,0.33}
\definecolor{newcolor}{rgb}{.8,.349,.1}

\newcommand{\hui}[1]{{\color{purple}#1}}
\newcommand{\huic}[1]{{\color{purple}[HH: #1]}}
\newcommand{\dc}[1]{{\color{red}#1}}
\newcommand{\dlc}[1]{{\color{brickred}[DL: #1]}}
\newcommand{\jyc}[1]{{\color{coral}[YJY: #1]}}
\newcommand{\jy}[1]{{\color{blue}#1}}



